Optical tomography: forward and inverse problems

This paper is a review of recent mathematical and computational advances in optical tomography. We discuss the physical foundations of forward models for light propagation on microscopic, mesoscopic and macroscopic scales. We also consider direct and numerical approaches to the inverse problems that arise at each of these scales. Finally, we outline future directions and open problems in the field.

==> Approximation_errors.tex <==
\subsection{Approximation errors\label{sect:approximation_errors}}

The model based approach is predicated on the implicit assumption
that there exists in principle an ``exact model'' given by the
physical description of the problem and the task is to develop a
computational technique that matches noiseless measured data within
an accuracy below the expected level of measurement error. In other
words, we assume that model inaccuracies are insignificant with
respect to experimental errors. However, the computational effort in
constructing a forward model of sufficient accuracy can be
prohibitive at best. In addition the physical model may have
shortcomings that lead to the data being outside the range of the
forward model (non-existence of solution).

In the {\em approximation error method} \cite{kaipio05} we abandon
the need to produce an ``exact model''. Instead,
%one accepts that the errors occur.
we attempt to determine the statistical
properties of the modelling errors and compensate for them by incorporating
them into the image reconstruction using a Bayesian approach.  The
steps involved in using the approximation error theory are i) the
construction and sampling of a prior, ii) the construction of a
mapping from coarse to fine models, iii) calculation of forward data
from the samples on both coarse and fine models, iv) statistical
estimation of the mean and covariance of the differences between
data from the coarse and fine models.  In \cite{arridge2006a} this technique
was shown to
result in reconstructed images using a relatively inaccurate forward
model that were of almost equal quality to those using a more
accurate forward model; the increase in computational efficiency was
an order of magnitude.


==> bayesian_methods.tex <==

\subsection{Inverse problems in Bayesian framework.}\label{subsec:bayes}

In the Bayesian approach, the inverse problems are viewed as  problems of statistical
inference. Hence, all variables are modelled as random variables, and measurements
are used to infer on the probability distribution of the parameter of primary interest.
% For the sake of defineteness, let us 
We assume that $\xn$ and $y$ are random variables
in finite dimensional spaces $\R^n$ and $\R^m$, respectively. Assume that their
joint probability distribution in $\R^n\times \R^m$ is absolutely continuous with
respect to the Lebesgue measure, and hence expressible in terms of a joint
probability density $\pi(\xn,y)$. The key identity relates the conditional probability
densities to the joint probability density,
\begin{equation}\label{joint}
 \pi(\xn,y) = \pi(\xn)\pi(y\mid \xn) =\pi(y)\pi(\xn \mid y),
\end{equation}
where the marginal probability densities are 
\[
 \pi(\xn)=\int_{\R^m}\pi(\xn,y) {\rm d}y,\quad \pi(y)=\int_{\R^n}\pi(\xn,y){\rm d}\xn.
\]
If $\xn$ is the variable to be estimated based on the observed values of $y$, we call
$\pi(\xn)$ the prior probability density and $\pi(y\mid \xn)$ the likelihood density.
In this framework, the solution of the inverse problem is the posterior probability
density $\pi(\xn \mid y)$ that according to (\ref{joint}) is
\begin{equation}\label{bayes}
\pi(\xn \mid y)=\frac{\pi(\xn)\pi(y\mid \xn)}{\pi (y)},\quad y=y_{\rm measured},
\end{equation}
which is the well known Bayes' formula. In particular, if the noise is additive and
the noise $e$ and the unknown $\xn$ are mutually independent, formula 
% (\ref{continuous}) 
(\ref{discretized}) 
leads to the likelihood density
\[
 \pi(y\mid \xn)=\pi_{\rm noise}(y-A_h (\xn)),
\]
where $\pi_{\rm noise}$ is the probability distribution of the noise $e$. A particular
but versatile special case is when $\xn$ and $e$ are mutually independent and
Gaussian,
\[
 \xn \sim {\mathcal N}(\xns,\xncov),\quad e\sim {\mathcal N}(e_*,\Gamma_e),
\]
where $\xns \in\R^n$ and $e_*\in\R^m$ are the means and 
the symmetric positive definite matrices $\xncov \in\R^{n\times n}$
and $\Gamma_e\in\R ^{m\times m}$ are the covariance matrices, respectively. In this case,
the posterior density (\ref{bayes}) becomes
\begin{equation}\label{independent noise}
\fl \pi(\xn \mid y)\propto {\rm exp}\left(-\frac 12 (\xn -\xns)^{\rm T}\xncov^{-1}(\xn - \xns)
-\frac 12 (y-A_h (\xn)-e_*)^{\rm T}\Gamma_e^{-1}(y-A_h (\xn)-e_*)\right).
\end{equation}
Observe that this equation applies only if $\xn$ and $e$ are mutually inddependent.
If this is not the case, no closed formula for the posterior density can be written.
A notable exception is when the mapping $A_h$ is linear, i.e., we have the linear
additive model
\[
 y = A_h \xn + e.
\]
In this case, the joint probability density is Gaussian, with mean and covariance
\[
\fl
{\rm E}
\left\{ \left( 
\begin{array}{c} 
\xn \\ y 
\end{array} 
\right) \right\} 
= \left(
\begin{array}{c} 
{\rm E}\big\{\xn \big\} \\ 
{\rm E}\big\{y\big\}
\end{array}
\right)  
=\left(\begin{array}{c} \xns \\
A_{h} \xns + e_*\end{array}\right),
\]
\[
\fl
 {\rm cov}\left(\begin{array}{c} \xn\\ y\end{array}\right) =  \left(\begin{array}{cc}
 \Gamma_{\xn} & \Gamma_{\xn y} \\ \Gamma_{y \xn} & \Gamma_y\end{array}\right)
 =  \left(\begin{array}{cc}
 \Gamma_{\xn} & \Gamma_{\xn}A_{h}^{\rm T} +\Gamma_{\xn e} \\ 
 A_{h}\Gamma_{\xn} +\Gamma_{e \xn} & A_{h} \Gamma_{\xn}A_{h}^{\rm T} + \Gamma_{\xn e}A_{h}^{\rm T}
+A_{h}\Gamma_{\xn e}+\Gamma_e \end{array}\right),
\]
where $\Gamma_{\xn}$, $\Gamma_y$ and $\Gamma_e$ denote the covariance matrices of the
random vectors $\xn$, $y$ and $e$, respectively,
and the double subindex notation such as
$\Gamma_{\xn y}$ means the cross covariance of $\xn$ and $y$ defined
as
\[
 \Gamma_{\xn y}={\rm E}\big\{\big(\xn -{\rm E}\big\{\xn \big\}\big)
\big(y-{\rm E}\big\{y\big\}\big)^{\rm T}
\big\}\in\R^{n\times m},
\]
and the other cross correlations correspondingly. The posterior density in this case is
is also Gaussian with mean and covariance
\begin{eqnarray}
{\rm E}\big\{\xn \mid y\big\} &=& \xns + \Gamma_{\xn y}\Gamma_y^{-1}(y - {\rm E}\big\{
y\big\})  \\
\cov(\xn \mid y) &=& \widetilde\Gamma_{\xn} 
\end{eqnarray}
where $\widetilde\Gamma_{\xn} = \Gamma_{\xn} - \Gamma_{\xn y}\Gamma_y^{-1}\Gamma_{y \xn}$
is the Schur complement of $\Gamma_{\xn}$.


==> priors.tex <==
\subsection{Priors}
\subsubsection{Choice of covariance}

Note that the matrices $\icvx$, $\icvy$ are covariances. Their entries represent a correlation between data samples or pixels. They act like convolutions on the untransformed vectors. On the other hand $\cvx$, $\cvy$ are sparse, representing the local relationship between neighbours. We could obtain either of these by for example
\begin{enumerate}
\item take specific sample images, create $\icvx$, form (it's a linear problem) $\icvy = \mA \icvx \mA\tr$.
\item measure lots of data, create $\icvy$.
\item Specify a Markov Random field $\cvx \equiv \mymat{\MRF}$
\item Specify a PDE $\cvx \equiv \nabla\tr { \diffusivity \nabla}$
\item Do row or column normalisation
\end{enumerate}


The last of these is the least principled. But it's very common !

Regularisation is required to ameliorate the effect of ill-posedness. 
In the classical setting it is formulated in terms of a penalty function
that biases a solution away from solutions possessing undresirable properties
such as high frequency noise. In the Bayesian setting it is formulated in terms
of a prior distribution of acceptable images. Development of appropriate 
priors seeks to improve the image reconstruction quality but priors are also
required to support the approximation error method.

Methods such as first-order Tikhonov (Phillips-Twomey),
Total Variation (TV), or Generalised Gaussian Markov Random Field
methods (GGMRF)\,\cite{bouman93} make statistical assumptions about
the distribution of edges. They pose assumptions about the regularity (e.g., smoothness) 
of the solution, the regularity being measured in terms of some norm of the solution and its differentials.
prior distributions and their derivatives for use in reconstruction.
In addition the ``lumpy background''
prior provides an effective method of
estimating information content of different imaging
systems\,\cite{pineda2006}.

Image processing
methods for computer vision offer a large set of techniques for
de-noising and segmentation based on anisotropic diffusion
processes\,\cite{acar94,geman84,rudin92a,vogel96}.
These techniques formulate directly a PDE for image flow, rather than
as the Euler equation of a variational form and can be considered more general.
These approaches can be incorporated into the
inverse problem using both descent based inversion algorithms,
and within a 
constrained reconstruction approach such as the ``all-at-once''
method\,\cite{haber2004a}.



More specific prior information can be incorporated if we assume that some approximate knowledge of the
objects such as shape topology and intra-region parameter regions is
available.
Examples are i) define region boundaries using a simple
parameterisation\cite{kolehmainen99a} and
draw the coefficients of the parameterisation from a Gaussian or beta
distribution; ii) define piecewise constant values for the finite
number of regions and draw these from a Gaussian or beta distribution;
iii) add structure variation using a Gibbs sampling scheme drawing from a local statistical prior.


Use of multimodality information provides another mechanism for defining priors.
Provided that it is possible to associate a quantitative value in
ne modality to that in another then the former could be used as a
first order Tikhonov prior for the latter; we refer to this type of
information as a (\emph{commensurate prior}). However this
association may not always be possible
so we need to consider methods that reconstruct the optical tomography data
when there is no simple relationship
between the numerical values in the optical reconstruction and the
associate modality.  We term this an {\em incommensurate} prior.  One
approach is to treat the mapping between values in one modality
and the other as a set of hidden variables which must be estimated
together with the reconstructed image. The effect of this will be to
estimate a reconstructed image which is most like the prior image in
an information theoretic sense.  The use of information theoretic
metrics as a constraint in image reconstruction has been employed in
only relatively few cases\,\cite{chen2005a} and never to our
knowledge in a nonlinear problem.

\input{structural_priors}

==> ptab.tex <==


\begin{tabular}{|l|l|}
%Space & Definition \\ \hline
& \\ \hline 
$\msset = \{\lambda_\ell, \ell = 1\ldots n_{\lambda}\} $ & set of spectral samples \\
${\bf c} = \{c_k, k = 1\ldots n_c\}$ & set of chromophores\\
${\bf \flph} = \{\flph_k, k = 1\ldots n_p\}$ & set of fluorophores\\
${\absspace}$ &   {space of absorbtion functions}\\
${\scaspace}$ &   {space of scattering functions}\\
${\fluspace}$ &   {space of fluorescence functions}\\
${\ltmspace}$ & {space of lifetime functions}\\
${\mcmespace} $ & space of multiple chromophores \\
${\mfpespace} $ & space of multiple flurophores \\
${\msabsspace} = \absspace$ & {space of multispectral  absorbtion functions}\\
${\msscaspace} = \scaspace$ & {space of multispectral scattering functions}\\
${\msfluspace} = \fluspace$ & {space of multispectral fluorescence functions}\\
${\msltmspace}= \ltmspace $ & {space of multispectral lifetime functions}\\
${\tabsspace} = \absspace\times [0,T]$ & {space of time varying absorbtion functions}\\
${\tscaspace} = \scaspace\times [0,T]$ & {space of time varying scattering functions}\\
${\tfluspace} = \fluspace\times [0,T]$ & {space of time varying fluorescence functions}\\
${\tltmspace} = \ltmspace\times [0,T]$ & {space of time varying lifetime functions}\\
${\tmcmespace} = \mcmespace\times [0,T]$ & {space of time varying chromophore functions}\\
${\tmfpespace} = \mfpespace\times [0,T]$ & {space of time varying flurophore functions}\\
\hline
\end{tabular}



==> structural_priors.tex <==



\subsubsection{Structural priors \label{sect:gen_tikh_reg}}



Consider now the multimodality DOT where we have the MRI or CT image as the reference image $\solfref$. In such a
case it is reasonable to assume that the local regularity of the optical images correlate spatially quite well with the 
local regularity in the reference image $\solfref$. In the structural priors, the idea is to modify the standard 
regularizer $\Psi(\solf)$, which penalizes the regularity of the solution uniformly and isotropically over the entire
image domain, to accomodate and reflect this prior information.
%
In the implementation of the structural priors, we consider a particular form of the functional $\Psi$
\begin{equation}
\Psi(\solf) = \alpha \int_{\domain}\psi\left(|\nabla \solf|_{\mymat{D}}\right)\rmd \r,\  \alpha > 0.
\label{eq:Psi_variational_D}
\end{equation}
where  $\psi$ is an image to image mapping and
\begin{equation}
| \nabla\solf|_{\mymat{D}} := \sqrt{(\nabla \solf)^{\mathrm{T}}  \mymat{D}(\r) \nabla\solf}
\end{equation}
where $\mymat{D}$ is a symmetric tensor function and $\alpha$ is a regularization parameter.


Using standard variational techniques we obtain 
\begin{equation}
\rPDE(\solf) = - \nabla^{\mathrm{T}}\diffusivity \mymat{D}(\r) \nabla
\end{equation}
where we have defined the \emph{diffusivity}
\begin{equation}
\diffusivity := \frac{\psi'\left(|\nabla\solf|_{\mymat{D}}\right)}{|\nabla \solf|_{\mymat{D}}} 
\end{equation}
%and we can interpret  $ \pfrech(\solf) $ as the \Frechet\, derivative of $\psi$ evaluated at $\solf$.

Choice of $\mymat{D}$ allows us to control the behaviour of the image update
according to prior information about the image structure~\cite{kaipio99a, douiri2006a}. For example, by
choosing $\psi (t) = t^2$ and
\begin{equation}
\mymat{D}(\r) = \mymat{I} - (1 + \| \nabla \solfref (\r) \|^2)^{-1}  \nabla \solfref (\r) \nabla \solfref (\r)\tr
\end{equation}
we arrive to the non-homogeneous anisotropic smoothness regularization that was presented in \cite{kaipio99a}. 
On the other hand, with the choices $\mymat{D}(\r) = \mymat{I}$ and $\psi (t) = t^2$ we would arrive at the standard
first-order Tikhonov regularization.

In \cite{arridge2008a} the form 
\begin{equation}
	\mymat{D} = \gamma(\solfref)\, \mymat{I}
\end{equation}
was used where $\solfref$ was a reference image, and $\gamma$ an edge-indicator
function taken to be
\begin{equation}
	\gamma(\solfref) = \exp \left\{ -\left[\frac{|\nabla\solfref |}{T_{{\rm ref}}}\right] \right\}
\label{eq:gammafunc}
\end{equation}
where $T_{{\rm ref}}$ is a threshold controlling the influence of the edges in $\solfref$.

